ASTER: Natural and Multi-language Unit Test Generation with LLMs

Implementing automated unit tests is an important but time-consuming activity in software development. To assist developers in this task, many techniques for automating unit test generation have been developed. However, despite this effort, usable tools exist for very few programming languages. Moreover, studies have found that automatically generated tests suffer poor readability and do not resemble developer-written tests. In this work, we present a rigorous investigation of how large language models (LLMs) can help bridge the gap. We describe a generic pipeline that incorporates static analysis to guide LLMs in generating compilable and high-coverage test cases. We illustrate how the pipeline can be applied to different programming languages, specifically Java and Python, and to complex software requiring environment mocking. We conducted an empirical study to assess the quality of the generated tests in terms of code coverage and test naturalness -- evaluating them on standard as well as enterprise Java applications and a large Python benchmark. Our results demonstrate that LLM-based test generation, when guided by static analysis, can be competitive with, and even outperform, state-of-the-art test-generation techniques in coverage achieved while also producing considerably more natural test cases that developers find easy to understand. We also present the results of a user study, conducted with 161 professional developers, that highlights the naturalness characteristics of the tests generated by our approach.

==> content/pygments.tex <==
\newcommand\at{@}
\newcommand\lb{[}
\newcommand\rb{]}
\newcommand\Red[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{#1}}}
\newcommand\red[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\grayline[1]{\textcolor[rgb]{0.4,0.4,0.4}{{#1}}}
\newcommand\gray[1]{\colorbox[rgb]{0.8,0.8,0.8}{{#1}}}
\newcommand\brown[1]{\textcolor[rgb]{0.55,0.27,0.07}{#1}}
\newcommand\orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{\textbf{#1}}}
\newcommand\Orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{{#1}}}
%\newcommand\green[1]{\textcolor[rgb]{0.42,0.56,0.14}{#1}}
\newcommand\lime[1]{\textcolor[rgb]{0.13,0.55,0.13}{{#1}}}
\newcommand\blue[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\blued[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1$\dag$}}}
\newcommand\ColorLine[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\javagreen[1]{\textcolor[rgb]{0.25,0.5,0.35}{{#1}}}
\newcommand\javadocblue[1]{\textcolor[rgb]{0.25,0.35,0.75}{{#1}}}
\newcommand\dkgreen[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\green[1]{\textcolor[rgb]{0.0,0.6,0}{#1}}
\newcommand\Green[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\Greenul[1]{\textcolor[rgb]{0.0,0.6,0}{{#1}}}
\newcommand\mauve[1]{\textcolor[rgb]{0.58,0.0,0.82}{{#1}}}
\newcommand\yellow[1]{\textcolor[rgb]{1,0.9,0.5}{{\bf #1}}}
\newcommand\lblue[1]{\colorbox[rgb]{0.87,1,1}{{#1}}}

\newcommand\PYbg[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbf[1]{\textcolor[rgb]{0.73,0.40,0.53}{\textbf{#1}}}
\newcommand\PYbe[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYbd[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYbc[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbb[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYba[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaJ[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaK[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaH[1]{\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{#1}}
\newcommand\PYaI[1]{\textcolor[rgb]{0.69,0.00,0.25}{#1}}
\newcommand\PYaN[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaO[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaL[1]{\textcolor[rgb]{0.73,0.73,0.73}{#1}}
\newcommand\PYaM[1]{\textcolor[rgb]{0.74,0.48,0.00}{#1}}
\newcommand\PYaB[1]{\textcolor[rgb]{0.00,0.25,0.82}{#1}}
\newcommand\PYaC[1]{\textcolor[rgb]{0.67,0.13,1.00}{#1}}
\newcommand\PYaA[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaF[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\PYaG[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaD[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaE[1]{\textcolor[rgb]{0.63,0.00,0.00}{#1}}
\newcommand\PYaZ[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaX[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaY[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaR[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaS[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaP[1]{\textcolor[rgb]{0.49,0.56,0.16}{#1}}
\newcommand\PYaQ[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaV[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaW[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaT[1]{\textcolor[rgb]{0.50,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaU[1]{\textcolor[rgb]{0.82,0.25,0.23}{\textbf{#1}}}
\newcommand\PYaj[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYak[1]{\textcolor[rgb]{0.73,0.40,0.53}{#1}}
\newcommand\PYah[1]{\textcolor[rgb]{0.63,0.63,0.00}{#1}}
\newcommand\PYai[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYan[1]{\textcolor[rgb]{0.67,0.13,1.00}{\textbf{#1}}}
\newcommand\PYao[1]{\textcolor[rgb]{0.73,0.40,0.13}{\textbf{#1}}}
\newcommand\PYal[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYam[1]{\textbf{#1}}
\newcommand\PYab[1]{\textit{#1}}
\newcommand\PYac[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaa[1]{\textcolor[rgb]{0.50,0.50,0.50}{#1}}
\newcommand\PYaf[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYag[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYad[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYae[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaz[1]{\textcolor[rgb]{0.00,0.63,0.00}{#1}}
\newcommand\PYax[1]{\textcolor[rgb]{0.60,0.60,0.60}{\textbf{#1}}}
\newcommand\PYay[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYar[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYas[1]{\textcolor[rgb]{0.73,0.13,0.13}{\textit{#1}}}
\newcommand\PYap[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaq[1]{\textcolor[rgb]{0.53,0.00,0.00}{#1}}
\newcommand\PYav[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaw[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYat[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYau[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}

\newcommand\merun[1]{\textcolor[rgb]{0.45,0.0,0.0}{#1}}
\newcommand\purple[1]{\textcolor[rgb]{0.22,0.0,0.44}{#1}}
\newcommand\javaKeyWord[1]{\textcolor[rgb]{0.38,0.03,0.58}{\tt \textbf{#1}}}

\definecolor{blueish}{RGB}{250, 250, 255}
\definecolor{greenish}{RGB}{250, 255, 250}
\definecolor{redish}{RGB}{255, 200, 200}


\definecolor{highlight}{RGB}{175, 255, 100}
% ---- Grays ----
\definecolor{gray01}{gray}{.98}
\definecolor{gray05}{gray}{0.95}
\definecolor{gray08}{gray}{0.92}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray18}{gray}{0.82}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray35}{gray}{0.65}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray45}{gray}{0.55}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray55}{gray}{0.45}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray65}{gray}{0.35}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray85}{gray}{0.15}
\definecolor{gray90}{gray}{0.10}
\definecolor{gray95}{gray}{0.05}

==> content/rq3.tex <==
% \input{tables/naturalness}

\begin{table}
  \centering
  \scriptsize
  \vspace{10pt}
  \setlength{\tabcolsep}{4pt}
 \caption{Mutation scores.}
 % \vspace{-5pt}
  \resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{App} & \textbf{CM} & \textbf{ES} & \textbf{GPT4} & \textbf{LL-70b} & \textbf{CL-34b} & \textbf{GR-34b} & \textbf{LL-8b} & \textbf{GR-8b} \\ \midrule
Commons CLI & -- & 60.0 & 29.7 & 33.7 & 24.3 & 30.7 & 22.3 & 26.7 \\ 
Commons Codec & -- & 75.0 & 35.0 & 30.3 & 24.7 & 25.3 & 31.0 & 29.3 \\
\midrule
CargoTracker & -- & 16.0 & 22.7 & 17.0 & 16.0 & 21.0 & 10.3 & 12.7 \\ 
DayTrader & -- & 5.0 & 17.3 & 10.3 & 9.0 & 10.7 & 13.7 & 12.0 \\ 
PetClinic & -- & -- & 9.7 & 11.3 & 9.5 & 8.7 & 7.0 & 7.0 \\ 
App X & -- & 1.0 & -- & 2.0 & 6.0 & 14.0 & 4.7 & 5.0 \\ 
\midrule
Python Dataset & 8.8 & - & 7.6 & 6.1 & 6.4 & 2.9 & 4.0 & 4.5 \\ \bottomrule
\end{tabular}
% \vskip 1pt

    }
    \label{table:mutation-coverage}\\
    \tiny CM: CodaMosa, ES: EvoSuite, GR: Granite, LL: Llama, CL: CodeLlama \\
Commons Compress and Commons JXPath are excluded due to failures in mutation analysis.
% \vspace{-10pt}
\end{table}%


\textit{1. Java applications:}
\label{subsubsec:rq3a}
Table~\ref{table:mutation-coverage} shows the mutation scores achieved by CodaMosa, EvoSuite, and \aster, indicating the effectiveness of each tool in detecting code mutations. For Java SE applications, EvoSuite consistently demonstrates superior performance (60\%-75\%), whereas \aster achieved 22.3\%--35.0\% mutation coverage. This is expected, as EvoSuite sets mutation goals during test generation and improves the tests to enhance mutation coverage, and indicates scope for improving LLM-based test generation with mutation-coverage goals.
Conversely, \aster outperforms EvoSuite consistently on the EE applications, which correlates with \aster's higher code coverage achieved on these applications than EvoSuite.
% EvoSuite relies on heuristics to generate test cases, which limits its effectiveness for the more complex and large-scale nature of JE applications (e.g., JE has more keyword extensions than SE).
% EvoSuite's performance drops down to 1\% to 16\%. While \aster's performance also dropped compared to the results on the Java SE applications, it still produced relatively consistent mutation coverage, ranging from 4.7\% to 22.7\%.



\textit{2. Python applications:}
\label{subsubsec:rq2c}
CodaMosa performed the best with 8.8\% mutation scores, followed by \aster with GPT-4, which achieved 7.6\% mutation coverage. Similar to EvoSuite, CodaMosa uses mutation coverage to evolve test cases during generation, thus benefiting from this approach. Overall, both tools achieve low mutation scores.
\begin{table}
\vspace{15pt}
  \centering
  \setlength{\tabcolsep}{4pt}
  \scriptsize
  \caption{Ablation results: coverage difference by excluding context during preprocessing and adding postprocessing steps.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrrr}
    \toprule
    & \multicolumn{7}{c}{\textbf{Preprocessing}} & \multicolumn{6}{c}{\textbf{Postprocessing}} \\
    \cmidrule{2-14}
    & \multicolumn{5}{c|}{\textbf{Java}} &  \multicolumn{2}{c|}{\textbf{Python}} &  \multicolumn{3}{c|}{\textbf{Java}}
    &  \multicolumn{3}{c}{\textbf{Python}}\\
    \textbf{Coverage} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{EAC}} & \multicolumn{1}{c}{\textbf{PM}} & \multicolumn{1}{c}{\textbf{AM}} & \multicolumn{1}{c|}{\textbf{NAC}} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c|}{\textbf{FS}} & \multicolumn{1}{c}{\textbf{CF}} & \multicolumn{1}{c}{\textbf{RF}} & \multicolumn{1}{c|}{\textbf{CA}}& \multicolumn{1}{c}{\textbf{CF}} & \multicolumn{1}{c}{\textbf{RF}} & \multicolumn{1}{c}{\textbf{CA}} 
     \bigstrut\\
      \midrule
      % \midrule
    % \textbf{Fixing success} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \cellcolor[rgb]{ 0,  0,  0}  \\

    % \midrule
    \textbf{Line} &    -13.3  &   -7.2   &  -8.5    &    -7.5  &-22.4& -17.0 &  -18.9   &    +11.9  &    +2.3  & +17.6&+20.3 & +4.3 & +20.1 \bigstrut\\
    % \midrule
    \textbf{Branch} &    -23.1  &   -26.1   &  -28.9    &   -21.3  &      -43.3&-8.9 &  -7.6&   +14.9   &   +2.4   & +26.3 & +10.9 & +1.1& +8.5\bigstrut\\
    % \midrule
    \textbf{Method} &   -9.9   &    -0.2  &    -3.0  &   -1.4   &   -14.8  &-10.6 &-8.9 &   +10.1   &  +1.6    &  +12.5&+13.1 & -0.3&+10.3\bigstrut\\
    \bottomrule
    \end{tabular}%
  \label{tb:ablationjava}}\\
  \vskip 3pt
  \tiny CS: Constructor, EAC: extend abstract class, PM: private methods, AM: auxiliary methods, NAC: no additional context, FS: few shot, CF: compilation error fix, RF: runtime error fix, CA: coverage augmentation. All data are in \%.
  % Preprocessing numbers represent coverage loss, whereas postprocessing numbers represent coverage gain.
  % \vspace{-16pt}
\end{table}%
% \aster achieved lower mutation scores on Python projects than Java projects.

\begin{findingBox}{6}{
EvoSuite achieves considerably higher mutation scores than \aster on Java SE applications due to its use of mutation-coverage goals during test generation, whereas \aster outperforms EvoSuite on the EE applications.
}\end{findingBox}

==> content/rq4.tex <==
% \input{tables/ablationjava}



Our approach performs test generation by including various contexts in the LLM prompts during preprocessing and performing the postprocessing steps. To investigate the effect of these steps, we conducted an ablation study using two Java applications (Commons CLI and PetClinic) and the Python dataset. We used Granite-34B, as it offers a good balance between size and competitiveness compared to other model. % The postprocessing results were calculated across all applications, with intermediate results stored during the experiments.




\textit{1. Java ablation:}
\label{subsubsec:rq4a}
In terms of preprocessing, the ablation removes: (1) the constructor chain details (\textsc{cs}), (2) non-abstract inherited methods (\textsc{eac}), (3) private method call details (\textsc{pm}), (4) signatures of auxiliary methods  (\textsc{am}), and (5) all of the context gathered through static analysis (\textsc{nac}). The \textsc{nac} configuration, thus, provides only the focal method body along with an instruction (e.g., ``Generate unit test cases for the following Java method'') . In each ablation configuration, we remove the context related to that configuration, keeping everything else intact, to understand the individual effect. For postprocessing, we measured coverage gains contributed by compilation error fix (\textsc{cf}), runtime error fix (\textsc{rf}), and coverage augmentation (\textsc{ca}).
Table~\ref{tb:ablationjava} presents results. we found that excluding all context (\textsc{nac}) leads to significant loss in coverage, with reductions of 43.3\% branch coverage. In terms of different types of contexts, \textsc{cs} has a larger effect across all coverage metrics, but the other context types also have considerable effect.

% \begin{table}[t]
%   \centering
%   \setlength{\tabcolsep}{5pt}
%   \scriptsize
%   \caption{\small Python ablation results: coverage difference by excluding context during preprocessing and adding postprocessing steps.}
%   \resizebox{.75\linewidth}{!}{
%     \begin{tabular}{lrrrrr}
%     \toprule
%     & \multicolumn{2}{c}{\textbf{Preprocessing}} & \multicolumn{3}{c}{\textbf{Postprocessing}} \\
%     \cmidrule{2-6}
%     \textbf{Coverage} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{FS}} & \multicolumn{1}{c}{\textbf{CF}} & \multicolumn{1}{c}{\textbf{RF}} & \multicolumn{1}{c}{\textbf{CA}} 
%      \bigstrut\\
%       % \midrule
%       \midrule
%     % \textbf{Fixing success} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \cellcolor[rgb]{ 0,  0,  0}  \\
%     % \midrule
%     \textbf{Line} &    -17.0\%   &   -18.9\%    &  +20.3\%     &    +4.3\%   &  +20.1\%   \bigstrut\\
%     % \midrule
%     \textbf{Branch} &    -8.9\%   &   -7.6\%    &  +10.9\%     &   +1.1\%   &     +8.5\% \bigstrut\\
%     % \midrule
%     \textbf{Method} &   -10.6\%    &    -8.9\%   &    +13.1\%   &   -0.3\%    &   +10.3\%  \bigstrut\\
%     \bottomrule
%     \end{tabular}%
%   \label{tb:ablationpython}}\\
%   \vskip 3pt
%    CS: Constructor, FS: few shot, CF: compilation error fix, RF: runtime error fix,\\ CA: coverage augmentation. 
%    % Preprocessing numbers represent coverage loss, whereas postprocessing numbers represent coverage gain.
% \end{table}%
Among the postprocessing steps, \textsc{ca} has the largest effect, leading to coverage gains of 26.3\% branch coverage. \textsc{cf} also provides notable improvement, with coverage gains of at least 10\% on all metrics. Conversely, \textsc{rf} has a small impact on coverage, at most 2.4\%. In general, assertion fixes in test cases would not be expected to have a large effect on coverage (as much of a test's coverage is typically achieved prior to reaching assert statements).
% , but there may be scope for improving this postprocessing step via better analysis and feedback.

\textit{2. Python ablation:}
\label{subsubsec:rq4b}
For Python ablation, we exclude constructor information (\textsc{cs}) and few-shot examples (\textsc{fs}) from the prompt, and perform similar evaluation for postprocessing step. \textsc{cs} and \textsc{fc} have a similar effect, with roughly the same loss in coverage across the metrics. The postprocessing results are similar to the Java result. 

\begin{findingBox}{7}{\aster's preprocessing steps to add relevant contexts to LLM prompts have a significant effect on coverage. \aster's postprocessing steps of compilation error fix and coverage augmentation result in significant coverage gains, while runtime error fix causes a small gain.
}\end{findingBox}


==> content/rq5.tex <==
% In this RQ, we evaluate the efficiency of LLM generated test case in terms of time, cost, and number of test cases generated. We want to understand how feasible LLM-assisted test generation is and which part of the pipeline future researches be focused on to make this process more affordable.

% \paragraph{Cost} To understand the cost of performing LLM-assisted test generation, we computed the number of input and output tokens. Based on an estimated number based on OpenAI~\cite{} documentation, which says that 1 token is roughly estimated to be 4 characters, we converted the total number of input and output characters to tokens. We found that for running all the experiments with 6 models with 8 datasets for Java, would cost $>$\$10,000 for each run based on the pricing model of OpenAI models. For each method, the average cost of LLM-assisted test generation is \$X. 

% \paragraph{Time}

% \paragraph{Number of test cases}

==> content/survey_figures.tex <==
\begin{figure*}[t]
    \centering
\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, ,width=\linewidth]{figures/qualtricsjava.pdf}
		\centering
		\caption{Java related results}
	\label{fig:surveyjava}
	\end{subfigure}%
 \hfill
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, ,width=\linewidth]{figures/qualtricspython.pdf}
		\centering
		\caption{Python related results}
	\label{fig:surveypython}
	\end{subfigure}%
    \caption{Survey results}
    \label{fig:surveyresult}
\end{figure*}

\begin{figure}[t]
    \centering
\includegraphics[width=0.8\linewidth]{figures/q18.pdf}
    \caption{Survey response regarding whether user will add similar test case to their suite.}
    \label{fig:surveyq18}
\end{figure}

==> content/todo.tex <==
Politics todo:
1. Name clearance
2. Dataset clearance
3. Prompt clearance
4. Models clearance (Gemini, Claude, Mistral Large)

==> listings/methodnaturalness.tex <==
\begin{figure}[t]
    \removelatexerror
    \begin{minipage}{0.5\textwidth}
    \begin{algorithm}[H]
        \scriptsize
        \SetAlgoLined
        \SetAlgoCaptionSeparator{:}
        \SetAlCapFnt{\small}
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \SetKwComment{Comment}{\smallskip$\triangleright$~}{}
        \SetKwFunction{methodnat}{ComputeMethodNameNaturalness}
        \SetKwFunction{focalclass}{identifyFocalClass}
        \SetKwFunction{focalmethod}{identifyFocalMethods}
        \SetKwProg{Fn}{Function}{:}{}
        \SetKw{identifyFocalClass}{identifyFocalClass}
        \SetKw{identifyFocalMethods}{identifyFocalMethods}
        \SetKw{tokenizecode}{tokenizeCode}
        \SetKw{closenesscore}{ClosenessScore}
  

        \Input{test case $t_c$, test file $t_f$.}
        \Output{Naturalness score $n_s$}
        
        \Fn{\methodnat}{
        score $\leftarrow$ 0
        \Comment{Identify focal classes}
        exact\_match $e_m$, close\_matches $c_m$ $\leftarrow$ \identifyFocalClass($t_f$)
        \Comment{If exact match has been found}
        \If{exact_match e_m}{
            focal_method f_m $\leftarrow$ \identifyFocalMethods($e_m$, $t_c$)
        }
        \Else{
            \ForEach{method \textbf{m} $\in$ $c_m$}{$f_m \leftarrow f_m \cup \identifyFocalMethods(m, t_c)$}
            }
        \ForEach{method $m$ $\in$ $f_m$}
        {
        \Comment{Check if test name contains focal method name}
        \If{$m$ $\in$ test\_method\_name $tmm$}{
            score = 1
        }
        }
        \Comment{Remove focal method from test name and tokenize the rest}
        tokens $t \leftarrow \tokenizecode(tmm)$
        
        score $\leftarrow$ (score + (\closenesscore($t$, $t_c$)))/2
        return $score$
        }
        \caption{\textbf{\small Compute method name naturalness}}
        \label{alg:method-name-naturalness}
    \end{algorithm}
    \end{minipage}
%\end{figure}
%\begin{figure}[!htp]
%\removelatexerror
    \begin{minipage}{0.5\textwidth}
    \begin{algorithm}[H]
    \scriptsize
        \SetAlgoLined
        \SetAlgoCaptionSeparator{:}
        \SetAlCapFnt{\small}
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \SetKwComment{Comment}{\smallskip$\triangleright$~}{}
        \SetKwFunction{methodnat}{ComputeVariableNameNaturalness}
        \SetKwFunction{focalclass}{identifyFocalClass}
        \SetKwFunction{focalmethod}{identifyFocalMethods}
        \SetKwProg{Fn}{Function}{:}{}
        \SetKw{identifyvariablereferenced}{getDeclaredAndReferencedVariables}
        \SetKw{getformalargument}{getFormalArgumentNames}
        \SetKw{getassigned}{getAllAssignments}
        \SetKw{closenesscore}{ClosenessScore}
  

        \Input{test case $t_c$, test file $t_f$, data structure types $D_T$.}
        \Output{Naturalness score $n_s$}
        
        \Fn{\methodnat}{
        score $\leftarrow$ 0
        \Comment{Get all the variables declared and referenced}
        variables V $\leftarrow$ \identifyvariablereferenced($t_c$,$t_f$)
        \ForEach{$v$ $\in$ $V$}
        {
            \Comment{closeness score w.r.t. formal parameters}
            $F_S$ $\leftarrow$ []
            
            \Comment{Get all the formal argument names where variable $v$ passed as parameter}
            formal argument names $F_A$ $\leftarrow$ \getformalargument($t_c$, $v$)
            
            \Comment{Find match with formal parameter names}
            \ForEach{$f$ $\in$ $F_A$}
            {
                $F_S$ $\leftarrow$ $\cup$ \closenesscore($v$, $f$)
            }
            
            \Comment{closeness score w.r.t assigned values}
            $A_S$ $\leftarrow$ []
        
            
            \Comment{Get all the right hand sides where the $v$ has been assigned (with def-use chain)}
            
            $A_v$ $\leftarrow$ \getassigned($t_c$, $v$)
            
            \ForEach{$a$ $\in$ $A_v$}
            {
                $A_S$ $\leftarrow$ $\cup$ \closenesscore($v$, $a$)
            }
            
            \Comment{If variable is of a data structure type}
            \If{v.type $\in$ $D_T$}
            {
                
                score $\leftarrow$ score + max(max($A_S$), max($F_S$))
            }
            \Else{
            score $\leftarrow$ score + max(\closenesscore($v$, $v.type$), max($F_S$), max($A_S$)
            }
            
        }
        return $score$/$V.length$
        }
        \caption{\textbf{\small Compute variable name naturalness}}
        \label{alg:variable-name-naturalness}
    \end{algorithm}
    \end{minipage}
\end{figure}

==> listings/mocking.tex <==
% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{figures/mockalgo.png}
% \caption{Identifying mockable fields, types, and methods.}
% \label{fig:mocking-algorithms}
% \end{figure}

\begin{figure}[t]
\centering
    \removelatexerror
    \vspace{0.03em}
    \removelatexerror
        \begin{algorithm}[H]
        \footnotesize
        \SetAlgoLined
        \SetAlgoCaptionSeparator{:}
        \SetAlCapFnt{\small}
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \SetKw{FormalParamTypes}{formalParamTypes}
        \SetKwComment{Comment}{\smallskip$\triangleright$~}{}
        \SetKwFunction{FParams}{IdentifyMockedFieldsAndParameterTypes}
        \SetKwProg{Fn}{Function}{:}{}
        \Input{focal method $f_m$, focal class $f_c$, mockable APIs $\mathcal{T}_{apis}$}
        \Output{Candidate mockable Types $\mathcal{T}_m$, and mockable Fields $\mathcal{F}_m$}
        \Fn{\FParams}{
        \Comment{Identify mockable fields.}
        \smallskip$\mathcal{F}_m, \mathcal{T}_m \leftarrow \emptyset, \emptyset$\;
            \ForEach{$f \in f_c.\text{fields}$}{
                \If{$f.\text{type} \in \mathcal{T}_{apis}$}{
                    $\mathcal{F}_m \leftarrow \mathcal{F}_m \cup \{f\}$\;
                    }
                    }
        \smallskip\Comment{Identify all mockable Types}
        $T \leftarrow \{f_c\} \cup {\FormalParamTypes(f_m)}$\;
        \smallskip\While{$T \neq \emptyset$}{
            $t \leftarrow T.\text{pop()}$\;
            $\mathcal{T}_m \leftarrow \mathcal{T}_m \cup \{t : t \in \mathcal{T}_{apis}\}$\;
            \ForEach{$c \in t.\text{constructors}$}{
                $T \leftarrow T \cup \FormalParamTypes(c)$\;
            }
            }
        }
        \smallskip\Return{$\mathcal{T}_m$, $\mathcal{F}_m$}\;
    %     \caption{\textbf{\small Identifying mockable Fields and Types}}
    %     \label{alg:mocked-parameters-and-fields}
    % \end{algorithm}%\vspace{-0.55em}
    % \begin{algorithm}[H]
        \footnotesize
        \SetAlgoLined
        \SetAlgoCaptionSeparator{:}
        \SetAlCapFnt{\small}
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \SetKwComment{Comment}{\smallskip$\triangleright$~}{}
        \SetKwFunction{FScope}{IdentifyMockingScope}
        \SetKwProg{Fn}{Function}{:}{}
        \SetKw{IsReachable}{isReachable}
        \SetKw{IsServiceEntryClass}{isServiceEntryClass}
        \SetKw{IsOverriden}{isOverriden}
        \SetKw{CallSites}{callSites}
        \SetKw{IsConstructor}{isConstructor}
        \SetKw{IsStatic}{isStatic}
        \SetKw{Type}{type}
        \SetKw{ReceiverType}{receiverType}

        \Input{focal method $f_m$, focal class $f_c$, and mockable types $\mathcal{T}_{apis}$.}
        \Output{Mockable constructor calls $\mathcal{M}_c$, static calls $\mathcal{M}_s$, API calls $\mathcal{M}_a$}
        \Fn{\FScope}{
        $S, \mathcal{M}_c, \mathcal{M}_s, \mathcal{M}_a \leftarrow \emptyset, \emptyset, \emptyset, \emptyset$;
        
        \smallskip\Comment{Add focal method and constructor to scope}
        $S \leftarrow S \cup \{f_m, f_c.\textit{constructors}\}$;    
        
        \smallskip\Comment{Add methods reachable from $f_m$ within $f_c$}
        $S \leftarrow S \cup  \{m \in f_c.\textit{methods} : \IsReachable(f_m, m)\}$;
        
        \smallskip\Comment{Add service entry class methods to scope}
        \If{${\IsServiceEntryClass}(f_c)$}{
            $S \leftarrow S \cup \{m \in f_c.\textit{methods} : \IsOverriden(m)\}$;
        }
        
        \Comment{Iterate over all callsites.}
        \ForEach{$\textbf{m} \in S$}{
            \ForEach{$cs \in \CallSites(\textbf{m})$}{
                % \smallskip\Comment{Callee is a constructor of mockable API}
                \uIf{$\IsConstructor(cs) \wedge cs.\text{type} \in \mathcal{T}_{apis}$}{
                    $\mathcal{M}_c \leftarrow \mathcal{M}_c \cup {cs}$;
                    }
                
                % \smallskip\Comment{Callee is a static method of mockable API}
                \uIf{$\IsStatic(cs) \wedge cs.\text{type} \in \mathcal{T}_{apis}$}{
                    $\mathcal{M}_s \leftarrow \mathcal{M}_s \cup {cs}$;
                    }
                
                % \smallskip\Comment{The receiver object of the callee is a mockable APIs}
                \uIf{$\ReceiverType(cs) \in \mathcal{T}_{apis}$}{
                    $\mathcal{M}_a \leftarrow \mathcal{M}_a \cup {cs}$;
                }
            }
        }
        \Return{$\mathcal{M}_c, \mathcal{M}_s, \mathcal{M}_a$};
        }
        \caption{\textbf{\small Identifying mockable fields, types, and scope}}
        \label{alg:mock-scope-identification}
        %\vspace{-5pt}
    \end{algorithm}
    % \vspace{-18pt}
\end{figure}


==> pygments.tex <==
\newcommand\at{@}
\newcommand\lb{[}
\newcommand\rb{]}
\newcommand\Red[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{#1}}}
\newcommand\red[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\grayline[1]{\textcolor[rgb]{0.4,0.4,0.4}{{#1}}}
\newcommand\gray[1]{\colorbox[rgb]{0.8,0.8,0.8}{{#1}}}
\newcommand\brown[1]{\textcolor[rgb]{0.55,0.27,0.07}{#1}}
\newcommand\orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{\textbf{#1}}}
\newcommand\Orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{{#1}}}
%\newcommand\green[1]{\textcolor[rgb]{0.42,0.56,0.14}{#1}}
\newcommand\lime[1]{\textcolor[rgb]{0.13,0.55,0.13}{{#1}}}
\newcommand\blue[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\blued[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1$\dag$}}}
\newcommand\ColorLine[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\javagreen[1]{\textcolor[rgb]{0.25,0.5,0.35}{{#1}}}
\newcommand\javadocblue[1]{\textcolor[rgb]{0.25,0.35,0.75}{{#1}}}
\newcommand\dkgreen[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\green[1]{\textcolor[rgb]{0.0,0.6,0}{#1}}
\newcommand\Green[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\Greenul[1]{\textcolor[rgb]{0.0,0.6,0}{{#1}}}
\newcommand\mauve[1]{\textcolor[rgb]{0.58,0.0,0.82}{{#1}}}
\newcommand\yellow[1]{\textcolor[rgb]{1,0.9,0.5}{{\bf #1}}}
\newcommand\lblue[1]{\colorbox[rgb]{0.87,1,1}{{#1}}}

\newcommand\PYbg[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbf[1]{\textcolor[rgb]{0.73,0.40,0.53}{\textbf{#1}}}
\newcommand\PYbe[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYbd[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYbc[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbb[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYba[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaJ[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaK[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaH[1]{\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{#1}}
\newcommand\PYaI[1]{\textcolor[rgb]{0.69,0.00,0.25}{#1}}
\newcommand\PYaN[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaO[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaL[1]{\textcolor[rgb]{0.73,0.73,0.73}{#1}}
\newcommand\PYaM[1]{\textcolor[rgb]{0.74,0.48,0.00}{#1}}
\newcommand\PYaB[1]{\textcolor[rgb]{0.00,0.25,0.82}{#1}}
\newcommand\PYaC[1]{\textcolor[rgb]{0.67,0.13,1.00}{#1}}
\newcommand\PYaA[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaF[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\PYaG[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaD[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaE[1]{\textcolor[rgb]{0.63,0.00,0.00}{#1}}
\newcommand\PYaZ[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaX[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaY[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaR[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaS[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaP[1]{\textcolor[rgb]{0.49,0.56,0.16}{#1}}
\newcommand\PYaQ[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaV[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaW[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaT[1]{\textcolor[rgb]{0.50,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaU[1]{\textcolor[rgb]{0.82,0.25,0.23}{\textbf{#1}}}
\newcommand\PYaj[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYak[1]{\textcolor[rgb]{0.73,0.40,0.53}{#1}}
\newcommand\PYah[1]{\textcolor[rgb]{0.63,0.63,0.00}{#1}}
\newcommand\PYai[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYan[1]{\textcolor[rgb]{0.67,0.13,1.00}{\textbf{#1}}}
\newcommand\PYao[1]{\textcolor[rgb]{0.73,0.40,0.13}{\textbf{#1}}}
\newcommand\PYal[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYam[1]{\textbf{#1}}
\newcommand\PYab[1]{\textit{#1}}
\newcommand\PYac[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaa[1]{\textcolor[rgb]{0.50,0.50,0.50}{#1}}
\newcommand\PYaf[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYag[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYad[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYae[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaz[1]{\textcolor[rgb]{0.00,0.63,0.00}{#1}}
\newcommand\PYax[1]{\textcolor[rgb]{0.60,0.60,0.60}{\textbf{#1}}}
\newcommand\PYay[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYar[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYas[1]{\textcolor[rgb]{0.73,0.13,0.13}{\textit{#1}}}
\newcommand\PYap[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaq[1]{\textcolor[rgb]{0.53,0.00,0.00}{#1}}
\newcommand\PYav[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaw[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYat[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYau[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}

\newcommand\merun[1]{\textcolor[rgb]{0.45,0.0,0.0}{#1}}
\newcommand\purple[1]{\textcolor[rgb]{0.22,0.0,0.44}{#1}}
\newcommand\javaKeyWord[1]{\textcolor[rgb]{0.38,0.03,0.58}{\tt \textbf{#1}}}

\definecolor{blueish}{RGB}{250, 250, 255}
\definecolor{greenish}{RGB}{250, 255, 250}
\definecolor{redish}{RGB}{255, 200, 200}


\definecolor{highlight}{RGB}{175, 255, 100}
% ---- Grays ----
\definecolor{gray01}{gray}{.98}
\definecolor{gray05}{gray}{0.95}
\definecolor{gray08}{gray}{0.92}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray18}{gray}{0.82}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray35}{gray}{0.65}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray45}{gray}{0.55}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray55}{gray}{0.45}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray65}{gray}{0.35}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray85}{gray}{0.15}
\definecolor{gray90}{gray}{0.10}
\definecolor{gray95}{gray}{0.05}

==> tables/ablationjava.tex <==
% Table generated by Excel2LaTeX from sheet 'Ablation'
\begin{table}[htbp]
  \centering
  \footnotesize
  \caption{Results from ablation study on Java projects}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrrrrr}
    \toprule
    \textbf{Stage} & \multicolumn{5}{c}{\textbf{Pre-processing}} & \multicolumn{3}{c}{\textbf{Post-processing}} \\
    \midrule
    \textbf{Coverage} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{EAC}} & \multicolumn{1}{c}{\textbf{PM}} & \multicolumn{1}{c}{\textbf{HM}} & \multicolumn{1}{c}{\textbf{NAC}} & \multicolumn{1}{c}{\textbf{CF}} & \multicolumn{1}{c}{\textbf{RF}} & \multicolumn{1}{c}{\textbf{CA}} 
     \bigstrut\\
      \midrule
      \midrule
    % \textbf{Fixing success} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \cellcolor[rgb]{ 0,  0,  0}  \\

    % \midrule
    \textbf{Line coverage} &    13.3\%   &   7.2\%    &  8.5\%     &    7.5\%   &  22.4\%     &    11.9\%   &    2.3\%   & 17.6\% \bigstrut\\
    \midrule
    \textbf{Branch coverage} &    23.1\%   &   26.1\%    &  28.9\%     &   21.3\%   &     43.3\%   &   14.9\%    &   2.4\%    & 26.3\% \bigstrut\\
    \midrule
    \textbf{Method coverage} &   9.9\%    &    0.2\%   &    3.0\%   &   1.4\%    &   14.8\%    &   10.1\%    &  1.6\%     &  12.5\%\bigstrut\\
    \bottomrule
    \end{tabular}%
  \label{tb:ablationjava}}\\
  CS: Constructor, EAC: extend abstract class, PM: private method, HM: \hl{helper methods}, NAC: no additional context, CF: compilation error fix, RF: runtime fix, CA: coverage augmentation. Pre-processing numbers are coverage loss \% by removing that particular details, whereas for post-processing, \% of coverage gain has been computed. \hl{add mocking ablation}
\end{table}%

\begin{table}[htbp]
  \centering
  \footnotesize
  \caption{Results from ablation study on Python projects}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Stage} & \multicolumn{2}{c}{\textbf{Pre-processing}} & \multicolumn{3}{c}{\textbf{Post-processing}} \\
    \midrule
    \textbf{Coverage} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{FS}} & \multicolumn{1}{c}{\textbf{CF}} & \multicolumn{1}{c}{\textbf{RF}} & \multicolumn{1}{c}{\textbf{CA}} 
     \bigstrut\\
      \midrule
      \midrule
    % \textbf{Fixing success} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \cellcolor[rgb]{ 0,  0,  0}  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \cellcolor[rgb]{ 0,  0,  0}  \\

    % \midrule
    \textbf{Line coverage} &    16.95\%   &   18.89\%    &  20.34\%     &    4.28\%   &  20.13\%   \bigstrut\\
    \midrule
    \textbf{Branch coverage} &    8.87\%   &   7.63\%    &  10.86\%     &   1.09\%   &     8.54\% \bigstrut\\
    \midrule
    \textbf{Method coverage} &   10.58\%    &    8.93\%   &    13.06\%   &   -0.24\%    &   10.28\%  \bigstrut\\
    \bottomrule
    \end{tabular}%
  \label{tb:ablationpython}}\\
  CS: Constructor, FS: few shot, CF: compilation error fix, RF: runtime fix, CA: coverage augmentation. Pre-processing numbers are coverage loss \% by removing that particular details, whereas for post-processing, \% of coverage gain has been computed.
\end{table}%

==> tables/naturalness.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table*}[htbp]
%   \centering
%   \caption{Automated analysis of test naturalness}
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{|c|c|r|r|r|r|r|r|r|r|}
%     \hline
%     \textbf{Dataset} & \textbf{Subject} & \multicolumn{1}{c|}{\textbf{AS}} & \multicolumn{1}{c|}{\textbf{PAS}} & \multicolumn{1}{c|}{\textbf{DA}} & \multicolumn{1}{c|}{\textbf{NA}} & \multicolumn{1}{c|}{\textbf{EA}} & \multicolumn{1}{c|}{\textbf{TMNN}} & \multicolumn{1}{c|}{\textbf{TVNN}} & \multicolumn{1}{c|}{\textbf{TMNC}} \\
%     \hline
%     \multirow{8}{*}{\textbf{Commons-CLI}} & \textbf{EvoSuite} & 18.15\% & 7.44\% & 0.00\% & 21.49\% & 27.22\% & 1.55\% & 47.59\% & 0.00\% \\
% \cline{2-10}          & \textbf{Developer} & 29.83\% & 33.93\% & 2.41\% & 10.84\% & 5.71\% & 24.97\% & 47.61\% & 13.88\% \\
% \cline{2-10}          & \textbf{GPT-4} & 15.92\% & 10.02\% & 0.00\% & 11.52\% & 4.70\% & 45.23\% & 63.20\% & 69.05\% \\
% \cline{2-10}          & \textbf{Llama3-70b} & 15.12\% & 13.67\% & 0.00\% & 15.90\% & 8.75\% & 41.24\% & 69.19\% & 60.00\% \\
% \cline{2-10}          & \textbf{CodeLlama-34b} & 17.84\% & 4.65\% & 0.00\% & 11.80\% & 6.28\% & 45.10\% & 72.22\% & 68.75\% \\
% \cline{2-10}          & \textbf{Granite-34b} & 17.42\% & 23.65\% & 0.00\% & 5.27\% & 1.97\% & 50.20\% & 72.63\% & 79.86\% \\
% \cline{2-10}          & \textbf{Llama3-8b} & 19.57\% & 36.52\% & 0.00\% & 7.00\% & 7.84\% & 46.08\% & 69.82\% & 71.71\% \\
% \cline{2-10}          & \textbf{Granite-8b} & 19.68\% & 18.79\% & 0.00\% & 15.44\% & 9.76\% & 35.78\% & 76.37\% & 46.87\% \\
%     \hline
%     \multirow{8}{*}{\textbf{Commons-Codec}} & \textbf{EvoSuite} & 15.78\% & 4.83\% & 0.00\% & 8.07\% & 37.44\% & 2.36\% & 35.00\% & 0.00\% \\
% \cline{2-10}          & \textbf{Developer} & 28.72\% & 54.24\% & 0.00\% & 7.98\% & 0.14\% & 33.43\% & 22.40\% & 24.69\% \\
% \cline{2-10}          & \textbf{GPT-4} & 19.12\% & 9.68\% & 0.00\% & 15.37\% & 1.79\% & 54.83\% & 38.91\% & 90.01\% \\
% \cline{2-10}          & \textbf{Llama3-70b} & 19.74\% & 8.69\% & 0.00\% & 22.43\% & 2.04\% & 51.86\% & 54.11\% & 85.39\% \\
% \cline{2-10}          & \textbf{CodeLlama-34b} & 17.76\% & 9.47\% & 0.00\% & 6.46\% & 2.90\% & 52.67\% & 42.32\% & 83.97\% \\
% \cline{2-10}          & \textbf{Granite-34b} & 18.13\% & 17.84\% & 0.00\% & 3.16\% & 2.05\% & 49.13\% & 44.40\% & 80.33\% \\
% \cline{2-10}          & \textbf{Llama3-8b} & 18.45\% & 21.16\% & 0.00\% & 2.93\% & 2.66\% & 51.04\% & 48.07\% & 84.13\% \\
% \cline{2-10}          & \textbf{Granite-8b} & 18.74\% & 12.63\% & 0.00\% & 7.14\% & 2.21\% & 48.84\% & 43.33\% & 80.63\% \\
%     \hline
%     \multirow{8}{*}{\textbf{Commons-Compress}} & \textbf{EvoSuite} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Developer} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{GPT-4} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Llama3-70b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{CodeLlama-34b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Granite-34b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Llama3-8b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Granite-8b} &       &       &       &       &       &       &       &  \\
%     \hline
%     \multirow{8}{*}{\textbf{Commons-JxPath}} & \textbf{EvoSuite} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Developer} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{GPT-4} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Llama3-70b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{CodeLlama-34b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Granite-34b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Llama3-8b} &       &       &       &       &       &       &       &  \\
% \cline{2-10}          & \textbf{Granite-8b} &       &       &       &       &       &       &       &  \\
%     \hline
%     \end{tabular}%
%     }
%   \label{tab:addlabel}%
%   *AS: Assertion simplicity, PAS: \% of tests with no assertions, DA: \% of tests with duplicate assertions, NA: \% of tests with null assertions, EA: \% of tests with exception-related assertions, TMNN: Test method name naturalness, TVNN: Test variable name naturalness, TMNC: \% of test names cover the focal method
% \end{table*}%


==> tables/rq1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[htbp]
  \footnotesize
  \centering
  \caption{ASTER with various models comparing with EvoSuite and developer-written test cases}
  
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    % \multirow{2}[4]{*}{\textbf{Dataset}} & \multirow{2}[4]{*}{\textbf{Approach Name}} & \multicolumn{4}{c|}{\textbf{ASTER}} \\
\textbf{Dataset} &     \textbf{Approach Name}     &        \textbf{Method} & \textbf{Branch} & \textbf{Instruction} & \textbf{Line} \\
    \hline
    \multirow{8}{*}{\textbf{Commons-CLI}} & ASTER + GPT-4 & 69.01 & 59.89 & 69.17 & 68.15 \\
\cline{2-6}          & ASTER Llama-3-70b & 74.93 & 64.19 & 74.87 & 73.55 \\
\cline{2-6}          & ASTER Codellama-34b & 75.28 & 54.49 & 70.12 & 66.96 \\
\cline{2-6}          & ASTER Granite 34b & 80.85 & 61.46 & 74.87 & 73.09 \\
\cline{2-6}          & ASTER Llama-3-8b & 70.25 & 49.74 & 65.64 & 62.81 \\
\cline{2-6}          & ASTER Granite-8b & 77.00 & 48.05 & 65.89 & 62.27 \\
\cline{2-6}          & EvoSuite & 92.01 & 63.07 & 76.86 & 81.06 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Commons-Codec}} & ASTER GPT-4 & 74.65 & 71.23 & 75.57 & 86.57 \\
\cline{2-6}          & ASTER Llama-3-70b & 72.90 & 68.83 & 73.84 & 86.42 \\
\cline{2-6}          & ASTER Codellama-34b & 72.69 & 62.95 & 71.84 & 84.52 \\
\cline{2-6}          & ASTER Granite 34b & 72.84 & 59.00 & 71.48 & 84.36 \\
\cline{2-6}          & ASTER Llama-3-8b & 73.29 & 65.20 & 73.48 & 85.96 \\
\cline{2-6}          & ASTER Granite-8b & 70.43 & 54.73 & 67.45 & 82.66 \\
\cline{2-6}          & EvoSuite & 85.88 & 83.20 & 92.61 & 85.76 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Commons-Compress}} & ASTER GPT-4 & 0     & 0     & 0     & 0 \\
\cline{2-6}          & ASTER Llama-3-70b & 44.71 & 21.97 & 29.57 & 29.1 \\
\cline{2-6}          & ASTER Codellama-34b & 40.45 & 17.23 & 24.1  & 25 \\
\cline{2-6}          & ASTER Granite 34b & 37.16 & 15.01 & 21.96 & 23.6 \\
\cline{2-6}          & ASTER Llama-3-8b & 39.72 & 15.93 & 23.7  & 26 \\
\cline{2-6}          & ASTER Granite-8b & 38.22 & 15.16 & 23.34 & 23.9 \\
\cline{2-6}          & EvoSuite & 37.56 & 21.04 & 26.49 & 25.07 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Commons-JxPath}} & ASTER GPT-4 & 58.505 & 28.43 & 38.685 & 39.5 \\
\cline{2-6}          & ASTER Llama-3-70b & 56.3  & 29.13 & 40.72 & 40.8 \\
\cline{2-6}          & ASTER Codellama-34b & 47.97 & 21.215 & 31.905 & 32.3 \\
\cline{2-6}          & ASTER Granite 34b & 53.29 & 22.005 & 34.835 & 35.5 \\
\cline{2-6}          & ASTER Llama-3-8b & 50.615 & 22.46 & 33.255 & 33.6 \\
\cline{2-6}          & ASTER Granite-8b & 48.06 & 18.91 & 29.505 & 30.7 \\
\cline{2-6}          & EvoSuite & 15.48 & 6.55  & 10.45 & 11.67 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Cargotracker}} & ASTER GPT-4 & \multicolumn{1}{r|}{46.62} & \multicolumn{1}{r|}{27.865} & \multicolumn{1}{r|}{37.83} & \multicolumn{1}{r|}{35.8} \\
\cline{2-6}          & ASTER Llama-3-70b & \multicolumn{1}{r|}{41.3} & \multicolumn{1}{r|}{23.145} & \multicolumn{1}{r|}{24.535} & \multicolumn{1}{r|}{22.7} \\
\cline{2-6}          & ASTER Codellama-34b & \multicolumn{1}{r|}{45.69} & \multicolumn{1}{r|}{19.1} & \multicolumn{1}{r|}{35.635} & \multicolumn{1}{r|}{33.2} \\
\cline{2-6}          & ASTER Granite 34b & \multicolumn{1}{r|}{55.49} & \multicolumn{1}{r|}{28.535} & \multicolumn{1}{r|}{42.85} & \multicolumn{1}{r|}{40.3} \\
\cline{2-6}          & ASTER Llama-3-8b & \multicolumn{1}{r|}{40.625} & \multicolumn{1}{r|}{19.775} & \multicolumn{1}{r|}{33.565} & \multicolumn{1}{r|}{31.2} \\
\cline{2-6}          & ASTER Granite-8b & \multicolumn{1}{r|}{42.905} & \multicolumn{1}{r|}{20.335} & \multicolumn{1}{r|}{34.58} & \multicolumn{1}{r|}{33} \\
\cline{2-6}          & EvoSuite & 55.98 & 28.54 & 31.76 & 32.66 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Daytrader-8}} & ASTER GPT-4 & 42.89 & 20.56 & 26.7  & 25.8 \\
\cline{2-6}          & ASTER Llama-3-70b & 43.715 & 17.435 & 23.605 & 22.4 \\
\cline{2-6}          & ASTER Codellama-34b & 42.155 & 12.5  & 21.905 & 19.9 \\
\cline{2-6}          & ASTER Granite 34b & 45.83 & 15.62 & 24.17 & 22.9 \\
\cline{2-6}          & ASTER Llama-3-8b & 42.765 & 13.86 & 23.085 & 21.7 \\
\cline{2-6}          & ASTER Granite-8b & 19.68 & 6.7   & 10.23 & 9.7 \\
\cline{2-6}          & EvoSuite & 32.82 & 9.92  & 15.82 & 16.31 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{PetClinic}} & ASTER GPT-4 & 55.55 & 20    & 37.455 & 32.7 \\
\cline{2-6}          & ASTER Llama-3-70b & 50    & 16.875 & 31.36 & 25.9 \\
\cline{2-6}          & ASTER Codellama-34b & 51.01 & 12.5  & 32.435 & 27.6 \\
\cline{2-6}          & ASTER Granite 34b & 54.54 & 15.625 & 35.3  & 30.9 \\
\cline{2-6}          & ASTER Llama-3-8b & 49.995 & 18.75 & 35.48 & 32.1 \\
\cline{2-6}          & ASTER Granite-8b & 46.99 & 15    & 28.315 & 24 \\
\cline{2-6}          & EvoSuite & -     & -     & -     & - \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
    \hline
    \multirow{8}{*}{\textbf{Proprietary App X}} & ASTER GPT-4 & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} \\
\cline{2-6}          & ASTER Llama-3-70b &       &       &       &  \\
\cline{2-6}          & ASTER Codellama-34b &       &       &       &  \\
\cline{2-6}          & ASTER Granite 34b &       &       &       &  \\
\cline{2-6}          & ASTER Llama-3-8b &       &       &       &  \\
\cline{2-6}          & ASTER Granite-8b &       &       &       &  \\
\cline{2-6}          & EvoSuite & 9.37  & 0.18  & 1.63  & 4.51 \\
\cline{2-6}          & Hand-written test case &       &       &       &  \\
\hline
\end{tabular}
  \label{tb:rq1llm}%
\end{table*}%


==> tables/rq1_non_llm.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
  \centering
  \footnotesize
  \caption{Coverage data for EvoSuite and developer-written test cases}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|r|r|r|r|}
    \hline
    \textbf{Dataset} & \textbf{Approach} & \multicolumn{1}{c|}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{Branch}} & \multicolumn{1}{c|}{\textbf{Instruction}} & \multicolumn{1}{c|}{\textbf{Line}} \\
    \hline
    \hline
    \multirow{2}{*}{Commons-CLI} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{Commons-Codec} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{Commons-Compress} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{Commons-JxPath} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{Daytrader-8} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{PetClinic} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \multirow{2}{*}{Proprietary App X} & EvoSuite &       &       &       &  \\
\cline{2-6}          & Handwriten Test Case &       &       &       &  \\
    \hline
    \end{tabular}%
    }
  \label{tb:rq1nonllm}%
\end{table}%

